Kernel Based Reconstruction for Generalized Graph Signal Processing

In generalized graph signal processing (GGSP), the signal associated with each vertex in a graph is an element from a Hilbert space. In this paper, we study GGSP signal reconstruction as a kernel ridge regression (KRR) problem. By devising an appropriate kernel, we show that this problem has a solution that can be evaluated in a distributed way. We interpret the problem and solution using both deterministic and Bayesian perspectives and link them to existing graph signal processing and GGSP frameworks. We then provide an online implementation via random Fourier features. Under the Bayesian framework, we investigate the statistical performance under the asymptotic sampling scheme. Finally, we validate our theory and methods on real-world datasets.

==> IEEE.bst.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%  IEEE.bst  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Bibliography Syle file for articles according to IEEE instructions
% balemi@aut.ee.ethz.ch     <22-JUN-93>
% modified from unsrt.bib. Contributions by Richard H. Roy

ENTRY
{ address
	author
	booktitle
	chapter
	edition
	editor
	howpublished
	institution
	journal
	key
	month
	note
	number
	organization
	pages
	publisher
	school
	series
	title
	type
	volume
	year
}
{}
{ label }

INTEGERS { output.state before.all mid.sentence after.sentence after.block }

FUNCTION {init.state.consts}
{ #0 'before.all :=
	#1 'mid.sentence :=
	#2 'after.sentence :=
	#3 'after.block :=
}

STRINGS { s t }

FUNCTION {output.nonnull}
{ 's :=
	output.state mid.sentence =
	{ ", " * write$ }
	{ output.state after.block =
		% next line commented out by rhr and changed to write comma
		%	{ add.period$ write$
			{ ", " * write$ 
				newline$
				"\newblock " write$
			}
			{ output.state before.all =
				'write$
				{ add.period$ " " * write$ }
				if$
			}
			if$
			mid.sentence 'output.state :=
		}
		if$
		s
	}
	
	FUNCTION {output}
	{ duplicate$ empty$
		'pop$
		'output.nonnull
		if$
	}
	
	FUNCTION {output.check}
	{ 't :=
		duplicate$ empty$
		{ pop$ "empty " t * " in " * cite$ * warning$ }
		'output.nonnull
		if$
	}
	
	FUNCTION {output.bibitem}
	{ newline$
		"\bibitem{" write$
			cite$ write$
			"}" write$
		newline$
		""
		before.all 'output.state :=
	}
	
	FUNCTION {fin.entry}
	{ add.period$
		write$
		newline$
	}
	
	% 5/24/89 rhr
	%  modified fin.entry function - prints note field after body of entry  
	%FUNCTION {fin.entry}
	%{ add.period$
		%  note empty$
		%    'write$
		%    { "\par\bgroup\parindent=0em  " * annote * "\par\egroup " * write$
			%    }
		%  if$
		%  newline$
		%}
	
	FUNCTION {new.block}
	{ output.state before.all =
		'skip$
		{ after.block 'output.state := }
		if$
	}
	
	% new block without terminating last block with a comma
	FUNCTION {new.ncblock}
	{
		write$ 
		newline$
		"\newblock "
		before.all 'output.state :=
	}
	
	FUNCTION {new.nccont}
	{
		write$ 
		" "
		before.all 'output.state :=
	}
	
	FUNCTION {new.sentence}
	{ output.state after.block =
		'skip$
		{ output.state before.all =
			'skip$
			{ after.sentence 'output.state := }
			if$
		}
		if$
	}
	
	FUNCTION {not}
	{   { #0 }
		{ #1 }
		if$
	}
	
	FUNCTION {and}
	{   'skip$
		{ pop$ #0 }
		if$
	}
	
	FUNCTION {or}
	{   { pop$ #1 }
		'skip$
		if$
	}
	
	FUNCTION {new.block.checka}
	{ empty$
		'skip$
		'new.block
		if$
	}
	
	FUNCTION {new.block.checkb}
	{ empty$
		swap$ empty$
		and
		'skip$
		'new.block
		if$
	}
	
	FUNCTION {new.sentence.checka}
	{ empty$
		'skip$
		'new.sentence
		if$
	}
	
	FUNCTION {new.sentence.checkb}
	{ empty$
		swap$ empty$
		and
		'skip$
		'new.sentence
		if$
	}
	
	FUNCTION {field.or.null}
	{ duplicate$ empty$
		{ pop$ "" }
		'skip$
		if$
	}
	
	FUNCTION {emphasize}
	{ duplicate$ empty$
		{ pop$ "" }
		{ "{\em " swap$ * "}" * }
		if$
	}
	
	FUNCTION {boldface}
	{ duplicate$ empty$
		{ pop$ "" }
		{ "{\bf " swap$ * "}" * }
		if$
	}
	
	%FUNCTION {boldface}
	%{ 's swap$ :=
		%  s "" =
		%    { "" }
		%    { "{\bf " s * "}" * }
		%  if$
		%}
	%
	INTEGERS { nameptr namesleft numnames }
	
	FUNCTION {format.names}
	{ 's :=
		#1 'nameptr :=
		s num.names$ 'numnames :=
		numnames 'namesleft :=
		{ namesleft #0 > }
		{ s nameptr "{ff~}{vv~}{ll}{, jj}" format.name$ 't :=
			nameptr #1 >
			{ namesleft #1 >
				{ ", " * t * }
				{ numnames #2 >
					{ "," * }
					'skip$
					if$
					t "others" =
					{ " et~al." * }
					{ " and " * t * }
					if$
				}
				if$
			}
			't
			if$
			nameptr #1 + 'nameptr :=
			namesleft #1 - 'namesleft :=
		}
		while$
	}
	
	FUNCTION {format.authors}
	{ author empty$
		{ "" }
		{ author format.names }
		if$
	}
	
	FUNCTION {format.editors}
	{ editor empty$
		{ "" }
		{ editor format.names
			editor num.names$ #1 >
			{ ", Eds." * }
			{ ", Ed." * }
			if$
		}
		if$
	}
	
	FUNCTION {format.title}
	{ title empty$
		{ "" }
		{ "``" title "t" change.case$ * }
		if$
	}
	
	FUNCTION {n.dashify}
	{ 't :=
		""
		{ t empty$ not }
		{ t #1 #1 substring$ "-" =
			{ t #1 #2 substring$ "--" = not
				{ "--" *
					t #2 global.max$ substring$ 't :=
				}
				{   { t #1 #1 substring$ "-" = }
					{ "-" *
						t #2 global.max$ substring$ 't :=
					}
					while$
				}
				if$
			}
			{ t #1 #1 substring$ *
				t #2 global.max$ substring$ 't :=
			}
			if$
		}
		while$
	}
	
	FUNCTION {format.date}
	{ year empty$
		{ month empty$
			{ "" }
			{ "there's a month but no year in " cite$ * warning$
				month
			}
			if$
		}
		{ month empty$
			'year
			{ month " " * year * }
			if$
		}
		if$
	}
	
	% FUNCTION {format.date}
	% { year empty$
		% 	'year 
		% 	{ " "  year * }
		%   if$
		% }
	
	FUNCTION {format.btitle}
	{ title emphasize
	}
	
	FUNCTION {tie.or.space.connect}
	{ duplicate$ text.length$ #3 <
		{ "~" }
		{ " " }
		if$
		swap$ * *
	}
	
	FUNCTION {either.or.check}
	{ empty$
		'pop$
		{ "can't use both " swap$ * " fields in " * cite$ * warning$ }
		if$
	}
	
	FUNCTION {format.bvolume}
	{ volume empty$
		{ "" }
		{ "vol." volume tie.or.space.connect
			series empty$
			'skip$
			{ " of " * series emphasize * }
			if$
			"volume and number" number either.or.check
		}
		if$
	}
	
	FUNCTION {format.number.series}
	{ volume empty$
		{ number empty$
			{ series field.or.null }
			{ output.state mid.sentence =
				{ "number" }
				{ "Number" }
				if$
				number tie.or.space.connect
				series empty$
				{ "there's a number but no series in " cite$ * warning$ }
				{ " in " * series * }
				if$
			}
			if$
		}
		{ "" }
		if$
	}
	
	FUNCTION {format.edition}
	{ edition empty$
		{ "" }
		{ output.state mid.sentence =
			{ edition "l" change.case$ " edition" * }
			{ edition "t" change.case$ " edition" * }
			if$
		}
		if$
	}
	
	INTEGERS { multiresult }
	
	FUNCTION {multi.page.check}
	{ 't :=
		#0 'multiresult :=
		{ multiresult not
			t empty$ not
			and
		}
		{ t #1 #1 substring$
			duplicate$ "-" =
			swap$ duplicate$ "," =
			swap$ "+" =
			or or
			{ #1 'multiresult := }
			{ t #2 global.max$ substring$ 't := }
			if$
		}
		while$
		multiresult
	}
	
	FUNCTION {format.pages}
	{ pages empty$
		{ "" }
		{ pages multi.page.check
			{ "pp." pages n.dashify tie.or.space.connect }
			{ "p." pages tie.or.space.connect }
			if$
		}
		if$
	}
	
	FUNCTION {format.vol.num.pages}
	{ 
		volume empty$
		{"" }
		{"vol. " volume *}
		if$
		number empty$
		'skip$
		{", no. " number * *}
		if$
		pages empty$
		'skip$
		{ duplicate$ empty$
			{ pop$ format.pages }
			{ ", pp. " * pages n.dashify * }
			if$
		}
		if$
	}
	
	%FUNCTION {format.vol.num.pages}
	%%boldface added 3/17/87 rhr
	%{ volume field.or.null boldface
		%  number empty$
		%    'skip$
		%    { "(" number * ")" * *
			%      volume empty$
			%	{ "there's a number but no volume in " cite$ * warning$ }
			%	'skip$
			%      if$
			%    }
		%  if$
		%  pages empty$
		%    'skip$
		%    { duplicate$ empty$
			%	{ pop$ format.pages }
			%	{ ":" * pages n.dashify * }
			%      if$
			%    }
		%  if$
		%}
	
	FUNCTION {format.chapter.pages}
	{ chapter empty$
		'format.pages
		{ type empty$
			{ "chapter" }
			{ type "l" change.case$ }
			if$
			chapter tie.or.space.connect
			pages empty$
			'skip$
			{ ", " * format.pages * }
			if$
		}
		if$
	}
	
	FUNCTION {format.in.ed.booktitle}
	{ booktitle empty$
		{ "" }
		{ editor empty$
			{ "in " booktitle emphasize * }
			{ "in "  booktitle emphasize *  ", " * format.editors * }
			if$
		}
		if$
	}
	
	FUNCTION {empty.misc.check}
	{ author empty$ title empty$ howpublished empty$
		month empty$ year empty$ note empty$
		and and and and and
		{ "all relevant fields are empty in " cite$ * warning$ }
		'skip$
		if$
	}
	
	FUNCTION {format.thesis.type}
	{ type empty$
		'skip$
		{ pop$
			type "t" change.case$
		}
		if$
	}
	
	FUNCTION {format.tr.number}
	{ type empty$
		{ "Tech. {R}ep." }
		'type
		if$
		number empty$
		{ "t" change.case$ }
		{ number tie.or.space.connect }
		if$
	}
	
	FUNCTION {format.article.crossref}
	{ key empty$
		{ journal empty$
			{ "need key or journal for " cite$ * " to crossref " * crossref *
				warning$
				""
			}
			{ "In {\em " journal * "\/}" * }
			if$
		}
		{ "In " key * }
		if$
		" \cite{" * crossref * "}" *
	}
	
	FUNCTION {format.crossref.editor}
	{ editor #1 "{vv~}{ll}" format.name$
		editor num.names$ duplicate$
		#2 >
		{ pop$ " et~al." * }
		{ #2 <
			'skip$
			{ editor #2 "{ff }{vv }{ll}{ jj}" format.name$ "others" =
				{ " et~al." * }
				{ " and " * editor #2 "{vv~}{ll}" format.name$ * }
				if$
			}
			if$
		}
		if$
	}
	
	FUNCTION {format.book.crossref}
	{ volume empty$
		{ "empty volume in " cite$ * "'s crossref of " * crossref * warning$
			"In "
		}
		{ "vol." volume tie.or.space.connect
			" of " *
		}
		if$
		editor empty$
		editor field.or.null author field.or.null =
		or
		{ key empty$
			{ series empty$
				{ "need editor, key, or series for " cite$ * " to crossref " *
					crossref * warning$
					"" *
				}
				{ "{\em " * series * "\/}" * }
				if$
			}
			{ key * }
			if$
		}
		{ format.crossref.editor * }
		if$
		" \cite{" * crossref * "}" *
	}
	
	FUNCTION {format.incoll.inproc.crossref}
	{ editor empty$
		editor field.or.null author field.or.null =
		or
		{ key empty$
			{ booktitle empty$
				{ "need editor, key, or booktitle for " cite$ * " to crossref " *
					crossref * warning$
					""
				}
				{ "In {\em " booktitle * "\/}" * }
				if$
			}
			{ "In " key * }
			if$
		}
		{ "In " format.crossref.editor * }
		if$
		" \cite{" * crossref * "}" *
	}
	
	FUNCTION {article}
	{ output.bibitem
		format.authors "author" output.check
		new.block
		format.title ",''" * "title" output.check
		new.ncblock
		crossref missing$
		{ journal emphasize "journal" output.check
			format.vol.num.pages output
			format.date "year" output.check
		}
		{ format.article.crossref output.nonnull
			format.pages output
		}
		if$
		new.block
		note output
		fin.entry
	}
	
	FUNCTION {book}
	{ output.bibitem
		author empty$
		{ format.editors "author and editor" output.check }
		{ format.authors output.nonnull
			crossref missing$
			{ "author and editor" editor either.or.check }
			'skip$
			if$
		}
		if$
		new.block
		format.btitle "title" output.check
		crossref missing$
		{ format.bvolume output
			new.block
			format.number.series output
			new.sentence
			publisher "publisher" output.check
			address output
		}
		{ new.block
			format.book.crossref output.nonnull
		}
		if$
		format.edition output
		format.date "year" output.check
		new.block
		note output
		fin.entry
	}
	
	FUNCTION {booklet}
	{ output.bibitem
		format.authors output
		new.block
		format.title ",''" * "title" output.check
		new.nccont
		howpublished address new.block.checkb
		howpublished output
		address output
		format.date output
		new.block
		note output
		fin.entry
	}
	
	FUNCTION {inbook}
	{ output.bibitem
		author empty$
		{ format.editors "author and editor" output.check }
		{ format.authors output.nonnull
			crossref missing$
			{ "author and editor" editor either.or.check }
			'skip$
			if$
		}
		if$
		new.block
		format.btitle "title" output.check
		crossref missing$
		{ format.bvolume output
			format.chapter.pages "chapter and pages" output.check
			new.block
			format.number.series output
			new.sentence
			publisher "publisher" output.check
			address output
		}
		{ format.chapter.pages "chapter and pages" output.check
			new.block
			format.book.crossref output.nonnull
		}
		if$
		format.edition output
		format.date "year" output.check
		new.block
		note output
		fin.entry
	}
	
	FUNCTION {incollection}
	{ output.bibitem
		format.authors "author" output.check
		new.block
		format.title ",''" * "title" output.check
		new.ncblock
		crossref missing$
		{ format.in.ed.booktitle "booktitle" output.check
			format.bvolume output
			format.number.series output
			format.chapter.pages output
			new.sentence
			publisher "publisher" output.check
			address output
			format.edition output
			format.date "year" output.check
		}
		{ format.incoll.inproc.crossref output.nonnull
			format.chapter.pages output
		}
		if$
		new.block
		note output
		fin.entry
	}
	
	FUNCTION {inproceedings}
	{ output.bibitem
		format.authors "author" output.check
		new.block
		format.title ",''" * "title" output.check
		new.ncblock
		crossref missing$
		{ format.in.ed.booktitle "booktitle" output.check
			address empty$
			{ organization publisher new.sentence.checkb
				organization output
				format.date "year" output.check
			}
			{ address output.nonnull
				format.date "year" output.check
				organization output
			}
			if$
			format.bvolume output
			format.number.series output
			format.pages output
			publisher output
		}
		{ format.incoll.inproc.crossref output.nonnull
			format.pages output
		}
		if$
		new.block
		note output
		fin.entry
	}
	
	FUNCTION {conference} { inproceedings }
	
	FUNCTION {manual}
	{ output.bibitem
		author empty$
		{ organization empty$
			'skip$
			{ organization output.nonnull
				address output
			}
			if$
		}
		{ format.authors output.nonnull }
		if$
		new.block
		format.btitle "title" output.check
		author empty$
		{ organization empty$
			{ address new.block.checka
				address output
			}
			'skip$
			if$
		}
		{ organization address new.block.checkb
			organization output
			address output
		}
		if$
		format.edition output
		format.date output
		new.block
		note output
		fin.entry
	}
	
	FUNCTION {mastersthesis}
	{ output.bibitem
		format.authors "author" output.check
		new.block
		format.title ",''" * "title" output.check
		new.ncblock
		"M.S. thesis" format.thesis.type output.nonnull
		school "school" output.check
		address output
		format.date "year" output.check
		new.block
		note output
		fin.entry
	}
	
	FUNCTION {misc}
	{ output.bibitem
		format.authors output
		title howpublished new.block.checkb
		format.title ",''" * output
		new.nccont
		howpublished new.block.checka
		howpublished output
		format.date output
		new.block
		note output
		fin.entry
		empty.misc.check
	}
	
	FUNCTION {phdthesis}
	{ output.bibitem
		format.authors "author" output.check
		new.block
		format.btitle "title" output.check
		new.block
		"Ph.D. thesis" format.thesis.type output.nonnull
		school "school" output.check
		address output
		format.date "year" output.check
		new.block
		note output
		fin.entry
	}
	
	FUNCTION {proceedings}
	{ output.bibitem
		editor empty$
		{ organization output }
		{ format.editors output.nonnull }
		if$
		new.block
		format.btitle "title" output.check
		format.bvolume output
		format.number.series output
		address empty$
		{ editor empty$
			{ publisher new.sentence.checka }
			{ organization publisher new.sentence.checkb
				organization output
			}
			if$
			publisher output
			format.date "year" output.check
		}
		{ address output.nonnull
			format.date "year" output.check
			new.sentence
			editor empty$
			'skip$
			{ organization output }
			if$
			publisher output
		}
		if$
		new.block
		note output
		fin.entry
	}
	
	FUNCTION {techreport}
	{ output.bibitem
		format.authors "author" output.check
		new.block
		format.title ",''" * "title" output.check
		new.ncblock
		format.tr.number output.nonnull
		institution "institution" output.check
		address output
		format.date "year" output.check
		new.block
		note output
		fin.entry
	}
	
	FUNCTION {unpublished}
	{ output.bibitem
		format.authors "author" output.check
		new.block
		format.title ",''" * "title" output.check
		new.ncblock
		note "note" output.check
		format.date output
		fin.entry
	}
	
	FUNCTION {default.type} { misc }
	
	MACRO {jan} {"Jan."}
	
	MACRO {feb} {"Feb."}
	
	MACRO {mar} {"Mar."}
	
	MACRO {apr} {"Apr."}
	
	MACRO {may} {"May"}
	
	MACRO {jun} {"June"}
	
	MACRO {jul} {"July"}
	
	MACRO {aug} {"Aug."}
	
	MACRO {sep} {"Sept."}
	
	MACRO {oct} {"Oct."}
	
	MACRO {nov} {"Nov."}
	
	MACRO {dec} {"Dec."}
	
	MACRO {acmcs} {"ACM Computing Surveys"}
	
	MACRO {acta} {"Acta Informatica"}
	
	MACRO {cacm} {"Communications of the ACM"}
	
	MACRO {ibmjrd} {"IBM Journal of Research and Development"}
	
	MACRO {ibmsj} {"IBM Systems Journal"}
	
	MACRO {ieeese} {"IEEE Transactions on Software Engineering"}
	
	MACRO {ieeetc} {"IEEE Transactions on Computers"}
	
	MACRO {ieeetcad}
	{"IEEE Transactions on Computer-Aided Design of Integrated Circuits"}
	
	MACRO {ipl} {"Information Processing Letters"}
	
	MACRO {jacm} {"Journal of the ACM"}
	
	MACRO {jcss} {"Journal of Computer and System Sciences"}
	
	MACRO {scp} {"Science of Computer Programming"}
	
	MACRO {sicomp} {"SIAM Journal on Computing"}
	
	MACRO {tocs} {"ACM Transactions on Computer Systems"}
	
	MACRO {tods} {"ACM Transactions on Database Systems"}
	
	MACRO {tog} {"ACM Transactions on Graphics"}
	
	MACRO {toms} {"ACM Transactions on Mathematical Software"}
	
	MACRO {toois} {"ACM Transactions on Office Information Systems"}
	
	MACRO {toplas} {"ACM Transactions on Programming Languages and Systems"}
	
	MACRO {tcs} {"Theoretical Computer Science"}
	
	READ
	
	STRINGS { longest.label }
	
	INTEGERS { number.label longest.label.width }
	
	FUNCTION {initialize.longest.label}
	{ "" 'longest.label :=
		#1 'number.label :=
		#0 'longest.label.width :=
	}
	
	FUNCTION {longest.label.pass}
	{ number.label int.to.str$ 'label :=
		number.label #1 + 'number.label :=
		label width$ longest.label.width >
		{ label 'longest.label :=
			label width$ 'longest.label.width :=
		}
		'skip$
		if$
	}
	
	EXECUTE {initialize.longest.label}
	
	ITERATE {longest.label.pass}
	
	FUNCTION {begin.bib}
	{ preamble$ empty$
		'skip$
		{ preamble$ write$ newline$ }
		if$
		"\begin{thebibliography}{"  longest.label  * "}" * write$ newline$
		}
		
		EXECUTE {begin.bib}
		
		EXECUTE {init.state.consts}
		
		ITERATE {call.type$}
		
		FUNCTION {end.bib}
		{ newline$
			"\end{thebibliography}" write$ newline$
	}
	
	EXECUTE {end.bib}
	
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%% End of IEEE.bst %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
